Near-Optimal Acceleration for Smooth $\ell_p$ / $\ell_q$ Nondual Convex First-Order Oracle Optimization

We study the optimization of convex objectives with $(L,\kappa-1)$-H\"older-continuous gradients in $\ell_q$ over $R B_p^d$, $1<\kappa\le 2$. (MG26) provides selectors with a movement bound for the problem of chasing high-dimensional convex nested sets for every $p<q$ and generally reduces Lipschitz convex optimization to bounds on the movement of selectors. We couple that movement with H\"older descent yielding a polynomial-runtime first-order method whose feasible output, in the high-dimensional regime $T\le d$ and for $p<\min\{q,2\}$, has error $$ \widetilde O_{\kappa,p,q}\!\left( \frac{LR^\kappa}{T^{\kappa(1+1/p-(1/q-1/2)_+)-1}} \right), $$ after $T$ queries to a first-order oracle, solving the COLT 2015 open problem of (Guz15), up to logarithmic factors. At $(p,q)=(1,2)$, the rate is $\widetilde{O}(LR^\kappa/T^{2\kappa-1})$, including $\widetilde{O}(LR^2/T^{3})$ cubic decay in the smooth case.

==> includes/definitions.tex <==
\usepackage{xparse}
\usepackage{xargs} %

\newcommand\newlink[2]{{\protect\hyperlink{#1}{\normalcolor #2}}}
\makeatletter
%
%
\def\Hy@raisedlink@left#1{%
    \ifvmode
        #1%
    \else
        \Hy@SaveSpaceFactor
        \llap{\smash{%
        \begingroup
            \let\HyperRaiseLinkLength\@tempdima
            \setlength\HyperRaiseLinkLength\HyperRaiseLinkDefault
            \HyperRaiseLinkHook
        \expandafter\endgroup
        \expandafter\raise\the\HyperRaiseLinkLength\hbox{%
            \Hy@RestoreSpaceFactor
            #1%
            \Hy@SaveSpaceFactor
        }%
        }}%
        \Hy@RestoreSpaceFactor
        \penalty\@M\hskip\z@
    \fi
}
\newcommand\newtarget[2]{\Hy@raisedlink@left{\hypertarget{#1}{}}#2}
\makeatother

\newcommand\linktoproof[1]{{\normalfont[{\hyperlink{proof:#1}{$\downarrow$}}]}}
%
\newcommand\linkofproof[1]{\textbf{of \cref{#1}. }\newtarget{proof:#1}}


\newcommand\zt[1]{\newlink{def:z_continuous}{z_{#1}}} 
\newcommand\ztdot[1]{\newlink{def:z_continuous}{\dot{z}_{#1}}}
\newcommand\xt[1]{\newlink{def:x_continuous}{x_{#1}}}
\newcommand\yt[1]{\newlink{def:y_continuous}{y_{#1}}}
\newcommand\xtdot[1]{\newlink{def:x_continuous}{\dot{x}_{#1}}}



\newcommand\T{\newlink{def:total_number_of_steps}{T}} 

\providecommand\set[1]{\{ #1 \}}
\newcommand\setl[1]{\left\{ #1 \right\}}
\newcommand\setsuch[2]{\{ #1 \mid #2  \}}
\newcommand\setsuchl[2]{\left\{ #1 \mid #2  \right\}}


\newcommand\xbara{\newlink{def:x_bar_a}{\bar{x}_{\aig[ ]}}}

%
\newcommand{\bigo}[1]{O( #1 )}
\newcommand{\bigol}[1]{O\left( #1 \right)}
\newcommand{\bigop}[2]{\newlink{def:big_O_p}{O_{#1}}( #2 )}
\newcommand{\bigopl}[2]{\newlink{def:big_O_p}{O_{#1}}\left( #2 \right)}
\newcommand{\bigolp}[2]{\bigopl{#1}{#2}}
\newcommand{\bigotilde}[1]{\newlink{def:big_O_tilde}{\widetilde{O}}( #1 )}
\newcommand{\bigotildel}[1]{\newlink{def:big_O_tilde}{\widetilde{O}}\left( #1 \right)}
\newcommand{\bigotildep}[2]{\newlink{def:big_O_p}{\widetilde{O}_{#1}}( #2 )} %
\newcommand{\bigotildepl}[2]{\newlink{def:big_O_p}{\widetilde{O}_{#1}}\left( #2 \right)}
\newcommand{\bigotildelp}[2]{\bigotildepl{#1}{#2}}
\newcommand{\bigomega}[1]{\Omega( #1 )}
\newcommand{\bigomegal}[1]{\Omega\left( #1 \right)}
\newcommand{\bigomegatilde}[1]{\newlink{def:big_O_tilde}{\widetilde{\Omega}}( #1 )}
\newcommand{\bigomegatildep}[2]{\newlink{def:big_O_p}{\widetilde{\Omega}_{#1}}( #2 )}
\newcommand{\bigomegatildelp}[2]{\newlink{def:big_O_p}{\widetilde{\Omega}_{#1}}\left( #2 \right)}
\newcommand{\bigomegatildepl}[2]{\bigomegatildelp{#1}{#2}}
\newcommand{\bigomegapl}[2]{\newlink{def:big_O_p}{\Omega_{#1}}\left( #2 \right)}
\newcommand{\bigomegalp}[2]{\bigomegapl{#1}{#2}}


%


%
%

\let\oldnu\nu
\renewcommand\nu{\newlink{def:hoelder_smoothness_exponent}{\oldnu}} %

\newcommand\err[1]{\newlink{def:err}{E_{#1}}}
\let\strikedL\L
\renewcommand\L{\newlink{def:hoelder_smoothness_constant}{L}} 
\newcommand\RR{\newlink{def:initial_distance_to_minimizer}{R}} 
\newcommand\f{\newlink{def:acc_sec_smooth_convex_function_f}{f}} 
\newcommand\Lip{\newlink{def:Lipschitzness_constant}{L}} 
\newcommand\linenemi[1][1=\psi, usedefault]{\newlink{def:line_in_nemirovskis_quasi_agd}{\Lambda_{#1}}}


\renewcommand\d{\mathrm{d}}

\newcommandx\regret[2][2= , usedefault]{\newlink{def:acc_sec_regret}{R_{#1}^{#2}}}

\newcommand\tauk[1]{\newlink{def:tau_k_interpolation_parameter_linear_coupling}{\tau_{#1}}}
\newcommandx*\Gt[1][1=t, usedefault]{\newlink{def:acc_sec_differentiable_gap_bound}{G_{#1}}}
\newcommandx*\Lt[1][1=t, usedefault]{\newlink{def:acc_sec_differentiable_lower_bound}{L_{#1}}}
\newcommandx*\Ut[1][1=t, usedefault]{\newlink{def:acc_sec_differentiable_upper_bound}{U_{#1}}}

\newcommandx*\etai[2][1=t, 2=, usedefault]{\newlink{def:acc_sec_sequence_of_lr_for_accelerated_rates}{\eta_{#1}^{#2}}}

%
\newcommandx*\aig[2][1=t, 2=, usedefault]{a_{#1}^{#2}} 



%
\newcommand*\circledaux[1]{\tikz[baseline=(char.base)]{
    \node[shape=circle,draw,inner sep=0.8pt] (char) {#1};}}

\NewDocumentCommand{\circled}{ m o }{%
    \IfNoValueTF{#2}{ \circledaux{#1} }{ \stackrel{\circledaux{#1}}{#2} }%
}

\newcommandx*\prox[1][1=, usedefault]{\newlink{def:proximal_operator}{\operatorname{prox}_{#1}}}
\newcommand\Prox{\newlink{def:set_of_all_prox_points}{\operatorname{Prox}}}

\newcommandx*\yktilde[1][1=k, usedefault]{\newlink{def:y_k_tilde}{\tilde{y}_{#1}}} 
%
%
%
%
%
\newcommandx*\xk[1][1=k, usedefault]{x_{#1}} 
\newcommandx*\yk[1][1=k, usedefault]{y_{#1}} 
\newcommandx*\zk[1][1=k, usedefault]{z_{#1}} 
\newcommandx*\Ak[2][1=k, 2=, usedefault]{A_{#1}^{#2}}
\newcommandx*\ak[2][1=k, 2=, usedefault]{a_{#1}^{#2}}

%


\newcommandx*\breg[1][1=\psi, usedefault]{\newlink{def:bregman}{D_{#1}}}
\newcommandx*\bregd[1][1=\psi^{\ast}, usedefault]{\newlink{def:bregman}{D_{#1}}} %
\newcommand\xast{\newlink{def:xast}{x^\ast}}


\usepackage{cancel}
%
\newcommand\Ccancel[2][black]{
    \let\OldcancelColor\CancelColor
    \renewcommand\CancelColor{\color{#1}}
    \cancel{#2}
    \renewcommand\CancelColor{\OldcancelColor}
}

\newcommand\OPT{\operatorname{OPT}} 
\newcommandx*\Rp[1][1=, usedefault]{\mathbb{R}_{\geq 0}}

\newcommand\smax[1]{\newlink{def:softmax}{\operatorname{smax}_{#1}}}
\newcommand\smaxn[2]{\newlink{def:partial_softmax}{\operatorname{smax}^{\leq #1}_{#2}}}
\newcommand\spann[1]{\operatorname{span}\{#1\}}
\newcommand\vol{\operatorname{vol}}
\newcommand\sign{\operatorname{sign}}
\newcommand\subgrad{\partial}
\newcommand\dualnumber[1]{\newlink{def:youngs_conjugate_number}{{#1}_\ast}}


\renewcommand\S[2]{\newlink{def:q_fold_smoothing}{\mathcal{S}^{(#1)}_{#2}}}
\newcommand\smoothing{\newlink{def:1_fold_smoothing}{S}}

\newcommand\elll[1]{\newlink{def:thing_minimized_in_the_lower_bound}{\ell_{#1}}}

\newcommand\hadnorm[1]{\newlink{def:Hadamard_norm}{\norm{#1}_{\operatorname{Had}}}}

\newcommand\subdiff{\newlink{def:subdifferential}{\partial}}
\newcommandx*\subdiffeps[2][1=\epsilon, 2=, usedefault]{\newlink{def:epsilon_subdifferential}{\partial^{#1}_{#2}}}

\newcommand\deltainexact{\newlink{def:delta_inexact}{\delta}}
\newcommand\p{\newlink{def:p_from_p_norm}{p}}
\renewcommand\r{\newlink{def:exponent_of_regularizers_unif_convexity}{r}}
\newcommand\m{\newlink{def:m_max_of_p_and_2}{m}}
\newcommand\q{\newlink{def:order_of_derivative_for_smoothness}{q}}
\newcommand\muUnif{\newlink{def:regularizers_unif_cvx_constant}{\mu}}

\newcommand\Unif{\mathcal{U}}
\newcommand\Sphere{\mathbb{S}}


\renewcommand\dim{\newlink{def:dimension}{\operatorname{dim}}} 
\newcommand\Rd{\R^{d}} 
\newcommand\NN{\mathbb{N}} 

\newcommand{\extR}{\newlink{def:extended_reals}{\overline{\R}}}

\newcommand\eventindicator[1]{\newlink{def:event_indicator_function}{\mathbb{I}_{\{#1\}}}}

\newcommand\indicator[1]{\newlink{def:indicator_function}{I}_{#1}}

\newcommandx*\ballnorm[2][1=\beta, 2=\norm{\cdot}, usedefault]{\newlink{def:ball_norm}{B^{#2}_{#1}}}


\newcommandx*\taylorf[2][1=q, 2=f, usedefault]{\newlink{def:qth_taylor_expansion}{#2_{#1}}}

\newcommandx*\M[1][1=, usedefault]{\newlink{def:non_euclidean_moreau_envelope}{M_{#1}}}

\newcommandx*\iproxoracle[1][1=, usedefault]{\newlink{def:inexact_proximal_oracle}{\mathcal{O}_{#1}}}
\newcommandx*\iproxoraclehat[1][1=, usedefault]{\newlink{def:generalized_inexact_proximal_oracle}{\widehat{\mathcal{O}}_{#1}}}


\newcommand\subdiffsqnorm[1]{\newlink{def:subdiff_of_squared_norm}{h_{#1}}}

%
%
%

\newcommand{\EE}{\mathbb{E}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\aff}{\operatorname{aff}}


\newcommand{\PP}{\mathbb{P}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\Bin}{\operatorname{Bin}}

\newcommand{\R}{\mathbb R}
\newcommand{\E}{\mathbb E}
\newcommand{\Prob}{\mathbb P}
\newcommand{\cL}{\mathcal L}
\newcommand{\cK}{\mathcal K}
\newcommand{\eps}{\varepsilon}
\newcommand{\defi}{\coloneqq}
\newcommand{\norm}[1]{\left\lVert #1\right\rVert}
\newcommand{\abs}[1]{\left\lvert #1\right\rvert}
\newcommand{\innp}[1]{\left\langle #1\right\rangle}
%
\providecommand{\set}[1]{}
\renewcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\1}{\mathbf 1}
\newcommand{\argmin}{\operatorname*{argmin}}
\newcommand{\argmax}{\operatorname*{argmax}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\Reg}{\operatorname{Reg}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\st}{\operatorname{st}}
\newcommand{\Q}{\mathcal Q}
\newcommand{\model}{m}

\DeclareMathOperator{\VC}{VC}


\newcommand\minmax{\operatorname{min\,max}} 
\newcommand\fatseq{\operatorname{fat}^{\operatorname{seq}}} 
\newcommand\lin{\operatorname{lin}} 
\newcommand\pair{\operatorname{pair}} 
\newcommand\sfat{\operatorname{sfat}} 
\newcommand\fat{\operatorname{fat}} 
\newcommand\tr{\operatorname{tr}} 
\newcommand\B{B} 

\newcommand{\cU}{\mathcal{U}}
\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\Rad}{\{\pm1\}}
\newcommand{\linf}{\ell_\infty}
\newcommand{\lone}{\ell_1}
\newcommand{\ltwo}{\ell_2}

\newcommand{\ip}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\Ball}{B}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\cO}{\mathcal O}
\newcommand{\wtO}{\widetilde{\mathcal O}}
\newcommand{\Prb}{\mathbb P}

\newcommand{\seq}{\text{seq}}

